WANDER: An Explainable Decision-Support Framework for HPC

High-performance computing (HPC) systems expose many interdependent configuration knobs that impact runtime, resource usage, power, and variability. Existing predictive tools model these outcomes, but do not support structured exploration, explanation, or guided reconfiguration. We present WANDER, a decision-support framework that synthesizes alternate configurations using counterfactual analysis aligned with user goals and constraints. We introduce a composite trade-off score that ranks suggestions based on prediction uncertainty, consistency between feature-target relationships using causal models, and similarity between feature distributions against historical data. To our knowledge, WANDER is the first such system to unify prediction, exploration, and explanation for HPC tuning under a common query interface. Across multiple datasets WANDER generates interpretable and trustworthy, human-readable alternatives that guide users to achieve their performance objectives.

==> Sections/causal.tex <==
% \tzi{too generic. revise.}
Structural Causal Models (SCMs) enable~\sysname to reason about how changes to system configurations influence performance outcomes beyond what correlations can capture. An SCM defines a set of variables (e.g., cores, memory, runtime) as a directed acyclic graph (DAG), where each variable is computed by a function of its causal parents and an exogenous noise term. These noise terms account for system randomness and unmeasured effects, such as scheduling delays or background contentions. In~\sysname, we use SCMs to evaluate whether a generated configuration is causally plausible, to quantify the sensitivity of performance to resource changes, and to identify which inputs most influence a target metric.

Through SCMs,~\sysname can simulate what happens when the value of a configuration parameter is changed. %we intervene—e.g., setting GPU count to 4—by modifying the corresponding equation while keeping the rest of the system intact. 
This lets us preserve realistic dependencies while exploring counterfactual scenarios. For linear models, we compute causal influence using path coefficients that reflect how much a change in input affects the output. In nonlinear cases, we use gradients to capture local sensitivity near a baseline configuration. This analysis is used in~\sysname to explain why a certain parameter matters and how much it contributes to observed variation in runtime, energy, or other metrics.

In practical terms, SCMs help us do three things. \banooqa{First, %we filter out any counterfactual or recommended configuration that violates known causal structure--such as changing interdependent parameters in isolation. Second, 
we generate explanations by computing causal attribution scores and reporting which features have the largest effect on a given outcome. %Third, 
Second, we perform uncertainty-aware validation by simulating what would happen under the same unobserved noise, ensuring that outputs remain consistent with past data. Third, we plot the median and standard deviations of the estimate effects of recommendations/suggestions alongside the median and standard deviations of the estimate effects of the data to verify that the causal estimates remain consistent and that no additional uncertainty has been introduced.}

Consider a simple HPC setup with variables \texttt{Cores}, \texttt{Mem}, and \texttt{Runtime}. If the DAG encodes that both cores and memory affect runtime, the structural equation for runtime might look like \( \texttt{Runtime} = \beta_{\text{core}} \cdot \texttt{Cores} + \beta_{\text{mem}} \cdot \texttt{Mem} + \epsilon \), where \( \epsilon \) captures background noise. Any configuration synthesized by~\sysname is valid only if it respects this relationship, stays within reasonable changes based on historical variation, and maintains the observed variability from the real system. These checks allow~\sysname to reject unrealistic recommendations, improve interpretability, and ensure that decision support outputs remain trustworthy and grounded in how the HPC system actually behaves.
% \tzi{SCM}
% Existing methods for evaluating counterfactuals and recommendations typically rely on predictive accuracy~\cite{}, distributional similarity~\cite{}, or even custom distance measures that compute subspace distance~\cite{banday2024perfgen}. However, these approaches lack mechanisms to verify whether the generated outputs are causally plausible. A recommendation may achieve the target performance in a predictive sense, but still violate known causal relationships in the system — for instance, by altering mutually dependent variables independently. To address this gap in evaluation methodology, we propose to leverage Structural Causal Models (SCMs)~\cite{} as a framework for evaluating the causal consistency of generated configurations. %By learning a causal graph from historical data, SCMs capture the directionality and dependencies between configuration parameters and performance metrics. 
% Mathematically, an SCM is defined as a tuple 
% \(
% \mathcal{M} = \langle {\mathcal{G}}, {\mathbf{f}}, {P_U} \rangle
% \), where $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ is a DAG representing the causal graph, $\mathbf{f} = \{f_i\}$ is a set of structural functions for each variable, $P_U$ is a distribution that models how likely it is that performance metrics will be affected by unobserved randomness. %Modeling this uncertainty explicitly allows us to reason not just about expected values, but about the distribution of possible outcomes given an intervention.

% % Explicitly modeling \( P_U \) allows us to simulate interventions while holding these noise factors fixed, enabling counterfactual reasoning about what would happen to the same job under a different configuration. This makes SCMs well-suited for evaluating and validating counterfactuals and recommendations in a causally coherent manner.



% %is a probability distribution over exogenous (noise) variables.
% % \vspace{0.2in}
% % \annotate[yshift=0.4em]{above,right}{graph}{Causal graph with nodes (variables) and edges (causal relations)}
% % \annotate[yshift=0.4em]{above,right}{struct_eqns}{Functions defining each variable based on its parents in the graph}
% % \annotate[yshift=0.4em]{above,right}{exog}{Unobserved factors accounting for randomness}


% %enable simulation of interventions (via do-calculus), where we can estimate the effect of setting a variable (e.g., \texttt{GPU=1}) while holding confounders constant. 
% SCM framework provides simulation capability that allows evaluating whether counterfactuals are causally consistent with known system behavior, and enables validating recommendations as configurations that are not seen in the data but should be feasible under the learned causal structure. %Compared to feature-space techniques such as DiCE, which optimize for outcome validity and diversity without explicit causal constraints, SCMs offer a principled way to assess and improve the trustworthiness of generated decisions. Moreover, combining both approaches allows us to explore trade-offs: DiCE offers search diversity, while SCM-based validation enforces structural realism. In this work, we use SCMs both to evaluate counterfactuals independently and to simulate interventions that support robust, interpretable recommendation generation.
% This principled approach enables an additional layer of stringent evaluation that improves the trustworthiness of~\sysname.


==> Sections/counterfactual.tex <==
Figure~\ref{fig:overview} illustrates that counterfactual analysis is the backbone that powers different types of queries. 
Counterfactual analysis enables users to reason about alternative %system behaviors 
behaviors by generating new configurations that minimally differ from a given baseline and that would lead to a different performance outcome. 
It uses a pre-trained predictive model $f: \mathcal{X} \rightarrow \mathcal{Y}$, which can estimate performance metrics given a configuration $\mathcal{X}$. Based on the formulation proposed by Wachter et al.~\cite{wachter2017counterfactual}, once trained, the model’s parameters are held fixed during counterfactual generation. This constraint ensures that any change in output is caused solely by changes in the input configuration. %—not by retraining or model drift.
While in this work, we choose XGBoost~\cite{chen2015xgboost,chen2016xgboost} to train the model from the input tabular data because XGBoost has been widely used successfully; the choice of the predictive model can be selected by the users.

Counterfactual analysis requires users to specify an original configuration $\mathcal{X}$, and a desired $y^*$ target performance constraint, which can be single or multi-objective. $\mathcal{X}'_i$ is a counterfactual configuration and $f(\mathcal{X}'_i)$ is the predicted value. If the user does not specify $\mathcal{y}^*$, then~\sysname assumes that the user wants to achieve an optimal value for the identified performance target metrics for the dataset in question (\tzi{or is this recommendation?}). Although, in the prototype implementation of~\sysname, we use counterfactual analysis as the synthesis engine for all types of queries, the backend synthesizer engine can be extended or replaced to deploy many other synthesis engines such as~\gls{llms}, Generative Adversarial Network~\cite{creswell2018generative}, among many others. The rationale is that with minor modification, counterfactual analysis can be used as the unified engine for generation. While counterfactual analysis is the most suitable tool for the Exploratory (both kinds) and Modification queries, other generative methods are incapable of serving these three types of queries. However, counterfactual analysis can be extended to ask the prescriptive queries by assuming either a random initial baseline configuration or \tzi{what else?}. Thus this tool provides a unified backend for all types of queries and our choice of the backend.

\subsubsection{Recommendation}
\label{sec:recommend}
\input{Sections/recommend}

\subsubsection{Exploratory Analysis}
\label{sec:exploratory}
Counterfactual analysis can be formulated as an optimization problem over the input space that balances \tzi{three} different objectives: (1) validity: each generated configuration $\mathbf{x}'_i$ must lead the model $f$ to predict the desired target $\mathbf{y}^*$; (2) proximity: the configuration should change only what is necessary; inputs should stay close to the original $\mathbf{x}$, making changes actionable; and (3) diversity: the set of counterfactuals should represent distinct adjustment strategies, not minor variations of the same one. Equation~\ref{eqn:cf_loss} mathematically presents the loss function that is minimized to identify $N$ alternate configurations, where $N$ is specified by users or by default~\sysname generates \tzi{$5$} counterfactuals. 
% At the heart of this process lies a trained predictive model, \( f: \mathcal{X} \rightarrow \mathcal{Y} \), which estimates performance metrics (e.g., runtime, energy) given a configuration \( \mathbf{x} \). Once trained, the model’s parameters are held fixed during counterfactual generation. This constraint ensures that any change in output is caused solely by changes in the input configuration—not by retraining or model drift. This aligns with the principle from Wachter et al.~\cite{wachter2017counterfactual}, where counterfactual reasoning is framed as an optimization over the input space:
\vspace{0.2in}
\begin{equation}
\footnotesize
\resizebox{\columnwidth}{!}{
\eqnmarkbox[Green]{cf_loss}{\{\mathbf{x}'_1, \ldots, \mathbf{x}'_N\}} = \arg\min_{\{\mathbf{x}'_i\}} \left[
% \sum_{i=1}^N \eqnmarkbox[WildStrawberry]{validity}{\mathcal{L}(f(\mathbf{x}'_i), \mathbf{y}^*)} +
\sum_{i=1}^N \eqnmarkbox[WildStrawberry]{validity}{\mathcal{L}_{\text{valid}}(f(\mathbf{x}'_i), \mathbf{y}^*)} +
% \sum_{i=1}^N \eqnmarkbox[WildStrawberry]{validity}{\frac{1}{N} \sum_{i=1}^{N} (f(\mathbf{x}'_i) - \mathbf{y}^*)^2} +
\lambda_1 \eqnmarkbox[YellowOrange]{proximity}{\mathcal{L}_{\text{prox}}(\mathbf{x}, \mathbf{x}'_i)} -
\lambda_2 \eqnmarkbox[RoyalBlue]{diversity}{diversity}%{\text{det}(K)}
\right]
}
\label{eqn:cf_loss}
\end{equation}
\annotate[yshift=0.7em]{above,right}{cf_loss}{Optimal counterfactual set}
\annotate[yshift=0.50em]{above,right}{validity}{Ensures prediction is close\\ to specified target}
\annotate[yshift=-0.2em,xshift=-0.0em]{below,left}{proximity}{Penalizes large deviations\\ from the given config}
\resizebox{\columnwidth}{!}{
\annotate[yshift=-0.3em]{below,left}{diversity}{Promotes\\ distinct solutions}
}

% \vspace{0.15in}
% \noindent The optimization balances three objectives:
% \begin{itemize}[leftmargin=1.5em]
%     \item \textbf{Validity:} Each generated configuration \( \mathbf{x}'_i \) must lead the model \( f \) to predict the desired target \( \mathbf{y}^* \).
%     \item \textbf{Proximity:} The configuration should change only what is necessary; inputs should stay close to the original \( \mathbf{x} \), making changes actionable.
%     \item \textbf{Diversity:} The set of counterfactuals should represent distinct adjustment strategies, not minor variations of the same one.
% \end{itemize}
Where, %\textbf{Prediction Loss:} This term 
prediction loss, $    \mathcal{L}_{\text{valid}}(f(\mathbf{x}'_i), \mathbf{y}^*) = \frac{1}{N} \sum_{i=1}^{N} (f(\mathbf{x}'_i) - \mathbf{y}^*)^2$, ensures that the predicted performance of each generated configuration closely matches the user-defined performance goal. Next, proximity loss, $\mathcal{L}_{\text{prox}}(\mathbf{x}, \mathbf{x}') = \sum_{k=1}^{d} \frac{|\mathbf{x}_k - \mathbf{x}'_k|}{\text{MAD}_k}$, penalizes unnecessary deviations from the original configuration to preserve realism and make suggestions actionable in practice. Here, each feature difference normalized by its Median Absolute Deviation (MAD) to account for variability across features and ensure scale-invariant comparisons. Finally, the diversity loss term, $    \text{diversity} = \text{det}(K), \quad K_{ij} = \frac{1}{1 + \|\mathbf{x}'_i - \mathbf{x}'_j\|}$, promotes variation among counterfactuals. It computes a similarity matrix \( K \), where each entry $K_{ij}$ is the pair-wise distance between counterfactuals. The determinant \( \det(K) \) quantifies how diverse the generated samples are, a higher values indicate that the counterfactuals are spread out. %, not clustered, and represent distinct configuration options.
% encourages the generation of distinct counterfactuals by penalizing redundancy. It constructs a similarity matrix \( K \) where each entry \( K_{ij} = \frac{1}{1 + \|x'_i - x'_j\|} \) captures how similar a pair of counterfactuals \( x'_i \) and \( x'_j \) are. The determinant of this matrix, \( \det(K) \), serves as a compact measure of spread--larger values imply that the counterfactuals span a wider and more varied space of configurations, thus offering users a diverse set of feasible alternatives.



% \vspace{0.15in}
% \paragraph*{Component Losses}
% \begin{enumerate}[leftmargin=1.5em]
%     \item \textbf{Prediction Loss:}
%     \begin{equation*}
%     \mathcal{L}_{\text{valid}} = \frac{1}{N} \sum_{i=1}^{N} (f(\mathbf{x}'_i) - \mathbf{y}^*)^2
%     \end{equation*}

%     \item \textbf{Proximity Loss:}
%     \begin{equation*}
%     \mathcal{L}_{\text{prox}}(\mathbf{x}, \mathbf{x}') = \sum_{k=1}^{d} \frac{|\mathbf{x}_k - \mathbf{x}'_k|}{\text{MAD}_k}
%     \end{equation*}
%     where MAD is the median absolute deviation, used to normalize changes across features with different scales.

%     \item \textbf{Diversity Term:}
%     \begin{equation*}
%     \text{diversity} = \text{det}(K), \quad K_{ij} = \frac{1}{1 + \|\mathbf{x}'_i - \mathbf{x}'_j\|}
%     \end{equation*}
%     Maximizing this kernel matrix determinant encourages dissimilar solutions.
% \end{enumerate}

% \vspace{0.3em}
% \subsection{Example: HPC Resource Optimization via Counterfactuals}

% Suppose a user wants to improve job runtime using alternative resource configurations.

% \begin{itemize}[leftmargin=1.5em]
%     \item \textbf{Original Configuration:} \( \mathbf{x} = \{ \texttt{cores} = 64,~ \texttt{memory} = 128~\text{GB} \} \), with \( f(\mathbf{x}) = 1.2 \) hours
%     \item \textbf{Target Outcome:} \( \mathbf{y}^* = 1.0 \) hour
%     \item \textbf{Constraints:} cores ≤ 72, memory ≤ 256 GB
%     \item \textbf{MAD:} cores = 16, memory = 32 GB
% \end{itemize}

% Using Equation~\ref{eqn:cf_loss}, \sysname generates:

% \begin{align*}
% \mathbf{x}'_1 &= \{68~\texttt{cores},~128~\texttt{GB}\} \quad \text{(add cores)} \\
% \mathbf{x}'_2 &= \{64~\texttt{cores},~144~\texttt{GB}\} \quad \text{(add memory)}
% \end{align*}

% \noindent These results are:
% \begin{itemize}[leftmargin=1.5em]
%     \item Predictively valid (\( f(\mathbf{x}') \leq 1.0 \) hr)
%     \item Close to the original (within 15\%)
%     \item Feasible under system constraints
%     \item Diverse in their strategies (different resources adjusted)
% \end{itemize}


% \subsection{Methodological Framework}
% Counterfactual analysis generates alternative configurations, which are diverse and feasible inputs that minimally differ from a given instance to achieve a specified performance goal. In~\sysname, counterfactual analysis is formulated as a constrained optimization problem that balances three competing objectives: prediction validity, input proximity, and solution diversity. 

% \vspace{0.15in} \begin{equation} \eqnmarkbox[GreenYellow]{cf_loss}{{\mathbf{x}'_1, \ldots, \mathbf{x}'N}} = \arg\min{{\mathbf{x}'i}} \left[ \sum{i=1}^N \eqnmarkbox[WildStrawberry]{validity}{\mathcal{L}(f(\mathbf{x}'i), \mathbf{y}^*)} + \lambda_1 \eqnmarkbox[YellowOrange]{proximity}{\mathcal{L}{\text{prox}}(\mathbf{x}, \mathbf{x}'_i)} - \lambda_2 \eqnmarkbox[RoyalBlue]{diversity}{\text{det}(K)} \right] \label{eqn:cf_loss} \end{equation}

% \annotate[yshift=0.4em]{above,right}{cf_loss}{Optimal counterfactual set} \annotate[yshift=0.6em]{above,right}{validity}{Ensures prediction meets target} \annotate[yshift=-1.2em,xshift=0.5em]{below,left}{proximity}{Penalizes large deviations from original} \annotate[yshift=0.5em]{above,left}{diversity}{Promotes distinct solutions via kernel matrix}

% \vspace{0.1in} \noindent \textbf{Where:} \begin{itemize}[leftmargin=1.5em] \item $f: \mathcal{X} \rightarrow \mathcal{Y}$ is the trained predictive model \item $\mathbf{x} \in \mathcal{X}$ is the original configuration \item $\mathbf{y}^* \in \mathcal{Y}$ is the desired performance vector \item $K_{ij} = \frac{1}{1 + |\mathbf{x}'_i - \mathbf{x}'_j|}$ is the similarity kernel used to encourage diversity \end{itemize}

% \paragraph*{Component Losses}

% \vspace{-0.25em} \begin{enumerate}[leftmargin=1.5em] \item \textbf{Validity:} Ensures generated configurations achieve the desired outcome. 
% \begin{equation} \mathcal{L}{\text{valid}} = \frac{1}{N} \sum{i=1}^{N} (f(\mathbf{x}'_i) - \mathbf{y}^)^2 
% \end{equation}

% \item \textbf{Proximity:} Measures deviation from the original input using MAD-normalized distance. \begin{equation*} \mathcal{L}{\text{prox}}(\mathbf{x}, \mathbf{x}') = \sum{k=1}^{d} \frac{|\mathbf{x}_k - \mathbf{x}'_k|}{\text{MAD}_k} \end{equation*}

% \item \textbf{Diversity:} Rewards diverse counterfactuals by maximizing the determinant of the similarity kernel. \begin{equation*} \text{diversity} = \text{det}(K), \quad K_{ij} = \frac{1}{1 + |\mathbf{x}'_i - \mathbf{x}'_j|} \end{equation*} \end{enumerate}

% \vspace{0.3em} \subsection{Example: HPC Resource Optimization via Counterfactuals}

% We consider an HPC job where the objective is to reduce execution time through configuration adjustments.

% \begin{itemize}[leftmargin=1.5em] \item \textbf{Original Configuration:} $\mathbf{x} = {\texttt{cores} = 64,~ \texttt{memory} = 128~\text{GB}}$ with $f(\mathbf{x}) = 1.2$ hours. \item \textbf{Target Outcome:} $\mathbf{y}^* = 1.0$ hour. \item \textbf{Constraints:} cores $\leq 72$, memory $\leq 256$ GB. \item \textbf{Normalization:} MAD${\texttt{cores}} = 16$, MAD${\texttt{memory}} = 32$ GB. \end{itemize}

% Applying the counterfactual formulation in Equation~\ref{eqn:cf_loss}, \sysname generates:

% \begin{align*} \mathbf{x}'_1 &= {68~\texttt{cores}, 128~\texttt{GB}} \quad \text{(increased CPU)} \ \mathbf{x}'_2 &= {64~\texttt{cores}, 144~\texttt{GB}} \quad \text{(increased memory)} \end{align*}

% \paragraph*{Interpretation:} \begin{itemize}[leftmargin=1.5em] \item Both candidates achieve $f(\mathbf{x}') \leq 1.0$ hour (validity). \item Changes are within 15% of the original (proximity). \item Solutions illustrate different resource strategies (diversity). \item All configurations comply with cluster constraints (feasibility). \end{itemize}

% \noindent This formulation forms the basis of~\sysname’s counterfactual engine and underpins the exploratory and modification queries used in operational decision-making.

% Counterfactual analysis~\cite{} enables users to explore alternative scenarios and understand how different outcomes could have occurred under different conditions. Such explorations increase trustworthiness, transparency, and make AI/ML models interpretable. Specifically,~\sysname leverages counterfactual analysis to propose hypothetical configurations based on a given configuration and a predictive model. Those hypothetical configurations show how minimal changes are needed to alter a model's decision. For instance, given a predictive model $f$ and an input feature vector $X$, the corresponding prediction of the given $x$ is $y' = f(x)$. The goal of a counterfactual generation engine is to generate $n$ meaningful counterfactual configurations $X'$ by perturbing specific features within this given input $X$. The modified output $X'$ is then provided back to the predictive model $f$; it yields a distinctly different output $y'' = f(x')$. This improves the given predictive model in four different ways: (1) We can evaluate the sensitivity and variability of a model by analyzing how small changes in $x$ can affect the output, (2) The transition from $x$ to $x'$ and the corresponding changes from $f(x)$ to $f(x')$ make the predictive model's decision-making process visible and understandable. (3) The adaptation from $x$ to $x'$ can define a narrative of how different outcomes can be achieved, which is interpretable for humans. (4) $x'$ offers actionable guidance on what might be done in real world scenarios. 

% Wachter et al.~\cite{wachter2017counterfactual} address the methodology for determining counterfactuals from a predictive model and given sample. The function $f_w$ represents a predictive model parameterized by weight $w$. The weights w are optimized during the training phase of the predictive model. In the process of generating counterfactuals, $f_w$ is used to evaluate how modifications of an input $x'$ alter the predicted outcome, generating a new target $y'$, keeping the $w$ parameter constant in the generation process. Constant $w$ ensures that changes in the prediction are solely from the adjustment to the given input to the predictive model. To express the minimality, they introduce a distance function $d(x_i, x')$ to quantify the divergence of $x'$ and $x_i$. A factor $\lambda$ is introduced to trade off the prediction and closeness to the original instance. The overall optimization algorithm is as follows:

% \begin{equation}
%     \arg \min_{x'} \max_\lambda (\lambda(f_w(x') - y')^2 + d(x_i, x'))
%     \label{eq:wachter}
% \end{equation}

% However, the equation ~\ref{eq:wachter} lacks some key aspects of counterfactual generation. We first assume that our pipeline is responsible for generating $N$ counterfactuals ${x_1, x_2, ... x_n}$ from the given sample $x$. To generate meaningful and actionable counterfactuals, (1) we need to include diversity in the generated counterfactuals so that the pipeline provided offers a variety of actionable configurations, (2) our goal is to minimize changes from the original sample so that they can be placed close to the desired range, (3) the suggested actionable configurations must be feasible with real-world constraints. 

% So the optimized loss function for the counterfactual generation pipeline will be:

% \begin{equation}
%     CF(x) = arg \min_{x1,x2, ..xn}(Loss + \lambda_{1} * Proximity + \lambda_{2} * Diversity)
% \end{equation}

% Where, Loss is computed from the actual loss of the given machine learning predictive model, $\lambda_1$ and $\lambda_2$ are both parameters to control the proximity and diversity.

% \begin{equation*}
%     Loss = \frac{1}{N} * \sum_{i=1}^{N} \mathcal{L(f(x_i), x)}
% \end{equation*}

% Proximity is how close the generated counterfactual configurations are to the given sample.

% \begin{equation*}
%     Proximity = \frac{1}{k} * \sum_{i=1}^{N} \Delta(x_i, x)
% \end{equation*}

% We calculate the diversity using the  determinant of the kernel matrix given the counterfactuals.

% \begin{equation*}
%     Diversity = \det(M) 
% \end{equation*}

% where 

% \begin{equation*}
%     M(i, j) = \frac{1}{1 + \Delta(x_i, x_j)}
% \end{equation*}



% % %
% % Counterfactual analysis simulates hypothetical changes to an existing configuration. Given an original configuration $\mathbf{x}$ and a target outcome $\mathbf{y}^*$, \sysname generates a new configuration $\mathbf{x}'$ that would lead to the desired outcome under the predictive model:

% % \begin{equation*}
% % \mathbf{x}' = \arg\min_{\mathbf{x}'} \left[ \mathcal{L}_{\text{pred}}(f(\mathbf{x}'), \mathbf{y}^*) + \lambda_1 \mathcal{L}_{\text{dist}}(\mathbf{x}, \mathbf{x}') \right]
% % \end{equation*}

% % Where $\mathcal{L}_{\text{pred}}$ penalizes deviation from the target outcome, and $\mathcal{L}_{\text{dist}}$ penalizes large changes to the original configuration.

% % To support deeper exploration, \sysname extends this to generate \emph{Top-K counterfactuals} and \emph{Pareto frontiers} across multiple objectives:

% % \begin{equation*}
% % \mathcal{L}_{\text{diverse}} = \lambda_1 \mathcal{L}_{\text{pred}} + \lambda_2 \mathcal{L}_{\text{dist}} + \lambda_3 \mathcal{L}_{\text{div}}(\{\mathbf{x}'_j\})
% % \end{equation*}

% % This loss promotes diversity among counterfactuals that all meet the performance target. \sysname uses this to explore trade-offs between objectives such as energy efficiency and runtime.

% % %%%%%%%%%%%%%%%%%%
% % Counterfactual reasoning addresses questions of the form ``What would the outcome have been if the value of a particular parameter had been set differently?" Formally, given an input configuration $x \in R^d$ and a predictive model 
% % $f : R^d \rightarrow R^k$, the goal is to find a perturbed configuration $x'$ such that the model prediction changes in a desired way--e.g., achieving a target performance value $y^*$.

% % \vspace{0.2in} 
% % \begin{equation*} 
% % \eqnmarkbox[Green]{cf_instance}{\mathbf{x}'} = \arg\min_{\mathbf{x}'} \left[ \eqnmarkbox[WildStrawberry]{pred_loss}{\mathcal{L}_{\text{pred}}(f(\mathbf{x}'), \mathbf{y}^*)} + \lambda_1 \eqnmarkbox[YellowOrange]{distance}{\mathcal{L}_{\text{dist}}(\mathbf{x}, \mathbf{x}')} \right] \end{equation*} %\vspace{0.2in}
% % \annotate[yshift=0.4em]{above,right}{cf_instance}{Counterfactual\\ configuration} \annotate[yshift=0.4em]{above,right}{pred_loss}{Loss measuring deviation\\ from target outcome} \annotate[yshift=-1.0em]{below,left}{distance}{Penalty for deviating\\ from original configuration}

% % \noindent This formulation captures both counterfactual generation and explanation: it identifies minimal, plausible changes to the input that would yield the desired outcome. An extension to this formulation is the generation of diverse counterfactuals--multiple distinct configurations that satisfy the same target but reveal different pathways to improvement. This involves augmenting the objective with a diversity term:

% % \vspace{0.2in} \begin{equation} \eqnmarkbox[Green]{cf_diverse_loss}{\mathcal{L}(\mathbf{x}, {\mathbf{x}'j})} = \lambda_1 \eqnmarkbox[WildStrawberry]{pred_term}{\mathcal{L}{\text{pred}}} + \lambda_2 \eqnmarkbox[OliveGreen]{dist_term}{\mathcal{L}{\text{dist}}} + \lambda_3 \eqnmarkbox[RoyalBlue]{div_term}{\mathcal{L}{\text{div}}} \label{eqn:counterfactual_diverse} 
% % \end{equation} 
% % \annotate[yshift=0.4em]{above,right}{cf_diverse_loss}{Loss for generating\\ diverse counterfactuals} \annotate[yshift=0.8em]{above,left}{pred_term}{Ensures target performance\\ is achieved} 
% % \annotate[yshift=0.4em]{below,right}{dist_term}{Maintains proximity to original} 
% % \annotate[yshift=-0.4em]{below,left}{div_term}{Promotes diversity\\ among candidates}

% % \noindent Together, these formulations enable the system to explain why certain changes improve performance by identifying multiple valid and interpretable feasible alternatives within user-specified constraints.

% % \tzi{@ankur -- please describe the math and underlying theory of what DiCE uses.}

\textbf{How to use:} An~\gls{hpc}-specific example to put counterfactual analysis to perspective would be of a user wanting to reduce the runtime of an~\gls{hpc} job. The user would specify in~\sysname that the original configuration uses $64$ cores and $128$~GB memory, resulting in a predicted runtime of 1.2 hours. The user specifies a performance target of $1.0$ hour and provides system constraints such as $cores \le 72$ and $memory \le 256~GB$. \sysname uses Equation~\ref{eqn:cf_loss} to generate two valid counterfactuals: (1) increase cores to $68$ while keeping memory fixed, or (2) increase memory to $144~GB$ while keeping cores unchanged. Both satisfy the performance goal, remain within allowed bounds, and reflect distinct resource allocation strategies.

Counterfactual analysis supports two query templates from Table~\ref{tab:query-taxonomy}. The user may ask an inverse optimization query such as \textit{``What changes would reduce runtime to 1 hour?"} Alternatively, they may ask a forward what-if query: \textit{``What would happen to runtime if I increase memory to 144~GB?"}.~\sysname can answer both queries using the same counterfactual generation methodology.

==> Sections/implementation.tex <==
% \subsection{System Overview}
% \sysname is a query-driven decision support system. Given a structured dataset consisting of input configurations and measured outcomes (e.g., power consumption, runtime),~\sysname supports two key decision-making services: %prediction, 
% what-if exploration, and recommendation. %These are accessed through formalized query templates that guide users in exploring “what-if” scenarios. 
% \sysname consists of four core components: (1) \texttt{data\_preprocessing} (2) \texttt{decision\_making} (does both counterfactual and recommendation) (3) \texttt{explanation} and (4) \texttt{evaluation} -- evaluates using SCM and quantifies uncertainty to estimate confidence intervals for outputs.~\sysname is developed as a modular and extensible framework where users can extend each component with their preferred methodology by specifying their code on the \texttt{config.yaml} file. The system outputs either (a) one recommendation or (b) top-K configurations that achieve user-defined objectives, both annotated with how confident the framework is. %plausibility and uncertainty scores.

% \begin{itemize}
%     \item \textbf{Explanation Module (Interpretability Support):} To improve transparency and usability, \sysname provides natural language explanations of its outputs. It describes the rationale behind recommended or counterfactual configurations and highlights which parameters most influence a target metric under the current setup.
% \end{itemize}
\sysname is implemented using Python and comprises modules shown in Figure~\ref{fig:overview}. The GUI is implemented using Streamlit; the config file's format is JSON.
\subsection{Data Preprocessing}

% Issues that are present in data sometimes and are addressed automatically before applying SEM
% \begin{itemize}
%     \item singular matrix - PCA, then L2 reg if issues persist
%     \item highly correlated features - dropping
%     \item zero or neg covariance matrix - adding a small value
% \end{itemize}

Before applying predictive modeling or causal analysis, \sysname performs a set of automated preprocessing steps to prepare HPC job data. These steps ensure numerical stability and statistical validity, particularly for downstream Structural Equation Modeling (SEM). The system automatically detects and resolves the following issues:

\begin{itemize}
    \item \textbf{Singular matrices:} When the covariance matrix is singular (non-invertible), Principal Component Analysis (PCA) is applied to reduce dimensionality. If singularity persists, L2 regularization is applied to stabilize model estimation.

    \item \textbf{Highly correlated features:} Features with high pairwise correlation (above a fixed threshold) are pruned to reduce multicollinearity and improve interpretability.

    \item \textbf{Zero or negative-definite covariance matrices:} A small positive constant is added to the diagonal to ensure the matrix is positive definite and invertible.
\end{itemize}

These preprocessing steps are implemented as modular pipelines and applied consistently across real and generated data. % to ensure consistency and fairness in evaluation.


% \subsection{Evaluation} Counterfactual generating models will be validated in the following ways: \begin{itemize}
%     \item Comparing an SEM models trained on real and synthesized datasets to look for estimation percentages within a fixed threshold.
%     \item using a predictive model trained on real dataset and predicting the target for synthesized data. MAPE calculated should be within the fixed threshold.
%     \item comparing causal graphs of the model trained on real dataset and counterfactuals.
% \end{itemize}
Each of these services is powered by shared backend modules—generative modeling, counterfactual optimization, and causal validation. 

% \subsection{Recommendation Engine}
% \tzi{how are we generating satisficing recommendation? This is where we can plug in the beGreat framework? @Banooqa? For the paper, we do not need to integrate, we can do it separately.}

% \subsection{Counterfactual Generator}
% The counterfactual module builds on the DiCE (Diverse Counterfactual Explanations) framework~\cite{}, adapted to support HPC-specific constraints. We use Python version XyZ, and PyTorch version XYZ. The generator can operate in batch mode for top-K generation. To ensure that all generated samples are valid, we implement rejection sampling strategy where the synthesizer can generate many options, however,~\sysname prunes the ones that fall outside of user specified ranges. \tzi{@ankur -- explain more how we ensure that the generated samples are within user specified range. What is the input to DiCE, and anything else that is implementation specific.}

% \subsection{Explanation Module}
% \tzi{@ankur, @banooqa -- how we are using causal model's importance value as input to the llm to describe the impact in natural language.}
% The system converts the output of the internal model into structured natural language, highlighting the input parameters that most influenced the resulting performance outcome. Attribution scores are derived from causal impact metrics discussed in the evaluation section, ensuring the explanation reflects not just correlations but underlying mechanisms. These scores are passed to an LLM-based generator that uses templated reasoning patterns to produce user-facing justifications. For example, in the PM-100 dataset, if a user attempts to reduce power consumption and the system recommends lowering the number of nodes from 32 to 16, the explanation would state: ``Reducing the number of nodes lowers total power consumption by decreasing the aggregate active hardware footprint, which was identified as the dominant factor contributing to power usage."
% \tzi{We need to provide a response template if we want to avoid criticism that the AI is going to say garbage or make it unclear etc.}


% \subsection{Evaluation Pipeline}
% \tzi{@banooqa -- check and update.}
% The evaluation framework includes three modules: SEM modeling using the `semopy` package, predictive validation using models from scikit-learn and PyTorch, and causal graph comparison using `pgmpy`. The SEM module learns structural coefficients from both real and generated data, then compares them statistically. For graph comparison, we use the Structural Hamming Distance metric to evaluate similarity. \tzi{What else are we doing -- building models using what input, what is being used for testing.}

% \subsection{User Interface and Query Templates}
% We implemented a graphical user interface using Streamlit~\cite{} to make \sysname accessible. The GUI supports interactive formulation of decision queries by guiding the user through structured input forms corresponding to the three services:

\begin{comment}
    \begin{itemize}
    \item \textbf{Recommendation:} The user specifies target metrics (e.g., ``minimize runtime'' or ``keep power below 250W''), optionally with priority weights or hard thresholds. The system converts this into a \emph{satisficing query}, where the goal is to return a configuration that satisfies all user-defined constraints rather than globally optimizing a single metric. Internally, this is formulated as a multi-objective constrained optimization problem. For instance, if the user selects ``runtime $\leq$ 10 minutes'' and ``power $\leq$ 250W'', the solver searches for any configuration in the feasible space that meets both thresholds, even if it is not the absolute fastest or most power-efficient. This approach supports more practical, constraint-aware decision-making.
    \item \textbf{Counterfactual:} The user selects a baseline configuration and a target outcome (e.g., ``reduce runtime by 10\%"). The system parses this into a constrained optimization problem.
    \item \textbf{Explanation:} The user selects a metric of interest and either a configuration or counterfactual.~\sysname generates a causal importance based explanation of why the model decided that a configuration is useful using natural language. \tzi{Making some stuff up, not sure what we are doing or if it is even done or not.}
\end{itemize}
\end{comment}

\tzi{need to add may be an example of the gui with a sample output for the running dataset.}


==> Sections/intro2.tex <==
\gls{hpc} systems are essential infrastructure for scientific advancement, powering large-scale simulations, data-intensive analyses, and modeling efforts across domains such as climate science, genomics, materials engineering, and astrophysics. These systems enable computations at scales that are otherwise infeasible due to the complexity and size of modern scientific workloads. However, effective utilization of~\gls{hpc} systems remains a challenge. As architectures become increasingly heterogeneous—with combinations of CPUs, GPUs, and specialized accelerators—operational decision-making becomes more complex. 

High-performance computing (HPC) systems expose numerous interdependent parameters (knobs) influencing metrics such as execution time, energy consumption, resource utilization, and run-to-run variability. These parameters form a high-dimensional configuration space with complex, nonlinear interactions. Prior studies have demonstrated that a seemingly optimal configuration can lead to performance variability as high as \(4\times\) under slightly different conditions~\cite{patki2019performance}. Consequently, performance in HPC is not a single point objective but a multi-objective, non-convex trade-off space. Traditional tuning, relying on expert intuition or extensive trial-and-error, struggles to navigate this complexity. Data-driven predictive models, such as GPTune~\cite{wu2021gptune} and OpenTuner~\cite{ansel2014opentuner}, alleviate some burden by selecting configurations from historical data. However, these ``black-box'' tools predominantly find singular optimal solutions, neglecting systematic exploration and interpretability, which users critically need to understand trade-offs and to confidently navigate HPC configuration choices.

Exploring hypothetical ``what-if" scenarios enables users to examine how configuration changes affect HPC performance metrics. Such analyses allow users to manage performance trade-offs, avoid configurations associated with anomalies or high variability, and select suitable alternatives for critical workloads. Existing frameworks like GPTune~\cite{wu2021gptune}, OpenTuner~\cite{ansel2014opentuner}, and ATF~\cite{rasley2016atf} primarily identify single optimal configurations, and do not systematically support alternative scenario exploration. Users typically rely on custom scripts or manual analysis, which can be labor-intensive and limited in scope. Additionally, the black-box nature of predictive models creates uncertainty about recommendation reliability, causing hesitation in adopting machine-generated configurations. Addressing this gap requires quantifying prediction uncertainties, validating configurations against historical causal patterns, and clearly communicating trade-offs.

To address these gaps, we propose~\sysname--\textit{What-if Analysis and Navigation for Decision-support with Explainable Reasoning}, an explainable, structured decision-support framework designed to enable systematic exploration of hypothetical configurations in HPC environments. At its core, \sysname synthesizes configurations minimally modified from user-specified baselines (called counterfactuals) to achieve desired performance goals or avoid undesirable outcomes. Unlike existing autotuning methods that output single, non-interpretable optimal configurations, \sysname explicitly supports exploratory queries such as ``Given an initial configuration, what would happen to runtime if I doubled the GPU count?" or ``Given an initial configuration, what minimal changes could prevent node failures due to memory exhaustion?"



==> Sections/query-tax2.tex <==
\begin{table}[t]
\begin{singlespacing}
\centering
\caption{Mapping of Decision-Support Query Types to HPC Use Cases}
\label{tab:query-taxonomy}
\resizebox{\columnwidth}{!}{
\begin{tabular}{p{0.22\linewidth} p{0.28\linewidth} p{0.26\linewidth} p{0.22\linewidth} p{0.2\linewidth}}
\toprule
\textbf{Query Type} & \textbf{Query Template} & \textbf{Example HPC Use Case} & \textbf{Example Features} & \textbf{Example Metrics} \\
\midrule

\textbf{Prescriptive Queries} & 
\textit{What values of \texttt{<configuration>} will ensure \texttt{<performance>} stays within \texttt{<constraint>}?} & 
Suggest settings for runtime < 30s and power < 80W & 
\texttt{num\_nodes}, \texttt{num\_gpus}, \texttt{freq\_req} & 
\texttt{runtime}, \texttt{cpu\_power\_consumption} \\

\textbf{Exploratory Queries} & 
\textit{If I change \texttt{<parameter>} to \texttt{<value>}, how will it affect \texttt{<metric>}?} & 
How does increasing node count from 2 to 4 affect runtime or variability? & 
\texttt{bandwidth}, \texttt{num\_nodes}, \texttt{flops} & 
\texttt{runtime}, \texttt{std(runtime)}, \texttt{energy\_usage} \\

\textbf{Modification Queries} & 
\textit{What changes to \texttt{<configuration>} would have prevented failure?} & 
Which memory request would avoid job failure due to node exhaustion? & 
\texttt{req\_mem}, \texttt{NNode}, \texttt{is\_gpu} & 
\texttt{State}, \texttt{ExitCode}, \texttt{waiting\_time} \\

\textbf{Explanation Queries} & 
\textit{Which parameters most influenced \texttt{<metric>} for this configuration?} & 
Why did bandwidth influence runtime variability most? & 
\texttt{mem\_bandwidth}, \texttt{num\_cores\_alloc} & 
\texttt{runtime}, \texttt{performance\_variation} \\

\bottomrule
\end{tabular}
}
\end{singlespacing}
\end{table}


==> Sections/query-tax3.tex <==
\begin{table*}[t]
\begin{singlespacing}
\centering
\caption{Mapping structured query grammar to representative HPC use cases, with example features and performance metrics from real datasets.}
\label{tab:query-taxonomy}
\resizebox{\textwidth}{!}{
\begin{tabular}{p{0.7in}p{3.0in}p{2.0in}p{1.3in}p{1.2in}}
\toprule
\textbf{Query Type} & \textbf{Query Template} & \textbf{Example HPC Use Case} & \textbf{Eg. Features} & \textbf{Eg. Metrics} \\
\midrule

Prescriptive & 
\texttt{RECOMMEND configurations TO achieve: <metric$\in$\{range\}> UNDER <constraints>} & How can I run my application to keep runtime under 30s and power below 80W given that the number of nodes must be under 1024? & 
\texttt{num\_nodes, num\_gpus, req\_mem} & 
\texttt{runtime, power} \\
\hline

Exploratory What-if & 
\texttt{WHAT-IF change to base configuration with~<feature~=~value>~EVALUATE effect on: <metric(s)>} & 
What would happen to runtime if I increase nodes from 2 to 4? & 
\texttt{num\_nodes, bandwidth} & 
\texttt{runtime, energy} \\
\hline

Exploratory optimization& 
\texttt{WHAT~changes to base configuration with~<feature=value>~WOULD achieve <metric(s) UNDER constraint(s)>} & 
What changes to the QoS=1 and num\_tasks=128 would reduce runtime variability to under 5\%? & 
\texttt{bandwidth, num\_tasks} & 
\texttt{runtime variability} \\
\hline

Modification & 
\texttt{CHANGE outcome from <${class\_label}_1 \rightarrow {class\_label}_2$> BY modifying base configuration with <feature=value>} & 
What config changes reduce job failure due to GPU exhaustion? & 
\texttt{req\_mem, is\_gpu, AllocCPUS} & 
\texttt{failure, anomaly} \\
\hline

% Explanation & 
% %\texttt{EXPLAIN influence on: <metric> FOR configuration: <features>} 
% No explicit query.~\sysname explains the quality, impact, and uncertainty of the suggestions.
% & 
% %Why did memory bandwidth increase runtime variability? 
% & 
% %\texttt{bandwidth, num\_nodes, mem\_alloc} 
% & 
% \texttt{runtime variability, power} \\
Explanation & 
\multicolumn{4}{c}{\parbox{\linewidth}{No explicit query.~\sysname explains the quality, impact, and uncertainty of the suggestions if other queries are performed. \\Otherwise,~\sysname presents the causal influences of the top $k$ features on a chosen performance metric.}}%No explicit query.~\sysname explains the quality, impact, and uncertainty of the suggestions if other queries are performed.\\ Otherwise,~\sysname presents the causal influences of the top $k$ features on a chosen performance metric.}
\\
\bottomrule
\end{tabular}
}
\end{singlespacing}
\end{table*}


==> Sections/query-tax4.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}
% \usepackage{rotating}

\begin{table*}[t]
\begin{singlespacing}
\centering
\caption{Mapping structured query grammar to representative HPC use cases, with example features and performance metrics from real datasets.}
\label{tab:query-taxonomy}
\resizebox{\textwidth}{!}{
\begin{tabular}{p{0.4in}p{0.7in}p{3.0in}p{2.0in}p{1.3in}p{1.2in}}
\toprule
\textbf{{Service}} & \textbf{Query Type} & \textbf{Query Template} & \textbf{Example HPC Use Case} & \textbf{Eg. Features} & \textbf{Eg. Metrics} \\
\midrule

& Prescriptive & 
\texttt{RECOMMEND configuration: <features> TO achieve: <target(s)> UNDER constraints: <constraints>} & 
How can I run my application to keep runtime under 30s and power below 80W? & 
\texttt{num\_nodes, num\_gpus, req\_mem} & 
\texttt{runtime, power} \\
\cline{2-6}

\multirow{4}{*}{\rotatebox[origin=c]{90}
{Generative}} 
& Exploratory What-if & 
\texttt{WHAT-IF change:~<feature~=~value>~EVALUATE effect on: <metric(s)>} & 
What would happen to runtime if I increase nodes from 2 to 4? & 
\texttt{num\_nodes, bandwidth} & 
\texttt{runtime, energy} \\
\cline{2-6}

& Exploratory Optimization & 
\texttt{WHAT~changes to:~<features>~WOULD achieve: <target(s)>} & 
What changes would reduce runtime variability to under 5\%? & 
\texttt{bandwidth, num\_tasks} & 
\texttt{runtime variability} \\
\cline{2-6}

& Modification & 
\texttt{CHANGE outcome: <failure> BY modifying: <features>} & 
What config changes reduce job failure due to GPU exhaustion? & 
\texttt{req\_mem, is\_gpu, AllocCPUS} & 
\texttt{failure, anomaly} \\
\hline

%\multirow{1}{*}{%\rotatebox[origin=c]{90}{Explanation}} 
%& 
\multicolumn{2}{c}{Explanation} & 
\multicolumn{4}{c}{\parbox{\linewidth}{No explicit query.~\sysname explains the quality, impact, and uncertainty of the suggestions if other queries are performed. Otherwise,~\sysname presents the causal influences of the top $k$ features on a chosen performance metric.}} \\
\bottomrule
\end{tabular}
}
\end{singlespacing}
\end{table*}


==> Sections/query-tax5.tex <==
\begin{table}[t]
\centering
\caption{Structured grammar templates and their semantics for each supported query type. Baseline inputs can be selected interactively or uploaded as JSON; ranges are specified using mathematical notation.}
\label{tab:query-taxonomy}
\resizebox{\columnwidth}{!}{
\begin{tabular}{p{1.1in}p{1.2in}p{1.5in}}
\toprule
\textbf{Query Type} & \textbf{Structured YAML Template} & \textbf{Interpretation of Inputs and Query Behavior} \\
\midrule

\textbf{Prescriptive (Recommendation)} &
\texttt{Type: Recommend} \newline
\texttt{Targets:} \newline
\quad \texttt{- runtime: < 30s} \newline
\quad \texttt{- power: < 80W} \newline
\texttt{Constraints:} \newline
\quad \texttt{- num\_nodes: >= 2} \newline
\quad \texttt{- num\_nodes: <= 1024} \newline
\quad \texttt{- 1 <= num\_gpus\_per\_node <= 4} &
Requires specifying performance objectives and configuration constraints. \newline
No baseline is needed or used. \newline
\textit{Behavior:} Searches feasible space to find configurations satisfying targets. \newline
\textit{Output:} A ranked list of satisfying configurations. \\

\hline

\textbf{Exploratory What-If} &
\texttt{Type: WhatIf} \newline
\texttt{Baseline: ./inputs/job001.json} \newline
\texttt{Modified:} \newline
\quad \texttt{- num\_nodes: 4} \newline
\texttt{Metrics:} \newline
\quad \texttt{- runtime} \newline
\quad \texttt{- power} &
Requires a baseline configuration and specific changes to features. \newline
Targets (performance metrics) are optional. \newline
\textit{Behavior:} Evaluates performance effect of proposed change. \newline
\textit{Output:} Predicted performance and natural language explanation of delta. \\

\hline

\textbf{Exploratory Optimization} &
\texttt{Type: InverseWhatIf} \newline
\texttt{Baseline: ./inputs/job002.json} \newline
\texttt{Targets:} \newline
\quad \texttt{- runtime: < 45s} \newline
\texttt{Constraints:} \newline
\quad \texttt{- qos: = 1} \newline
\quad \texttt{- num\_tasks: = 128} &
Requires a baseline, target outcomes, and fixed constraints. \newline
\textit{Behavior:} Performs counterfactual optimization to discover minimal changes. \newline
\textit{Output:} A diverse set of feasible alternate configurations with trade-off scores. \\

\hline

\textbf{Modification (Failure Avoidance)} &
\texttt{Type: Modify} \newline
\texttt{Baseline: ./inputs/failing\_job.json} \newline
\texttt{TargetOutcome: success} &
Requires a baseline configuration and a binary outcome transition. \newline
\textit{Behavior:} Identifies the smallest change needed to flip model output (e.g., from failure to success). \newline
\textit{Output:} Actionable counterfactuals that prevent failures. \\

\hline

\textbf{Explanation} &
\texttt{Type: Explain} \newline
\texttt{Baseline: ./inputs/job003.json} \newline
\texttt{Metric: runtime} &
Requires a configuration and a target performance metric. \newline
\textit{Behavior:} Computes feature attribution or causal influence scores. \newline
\textit{Output:} List of most influential features, sensitivity analysis, and causal diagnostics. \\

\bottomrule
\end{tabular}
}
\end{table}


==> Sections/recommend.tex <==
\tzi{If we are using counterfactuals for this -- we need to describe differently.}
Recommendation queries begin with a set of performance goals (e.g., minimize runtime, reduce power) and return a configuration that satisfies these goals without requiring a baseline configuration. \sysname formulates this as a satisficing optimization problem over the feasible configuration space $\mathcal{C} \subseteq \mathbb{R}^d$:

\begin{equation*}
\mathbf{x}^* = \arg\min_{\mathbf{x}' \in \mathcal{C}} \mathcal{L}_{\text{multi}}(f(\mathbf{x}'), \mathbf{y}^*)
\end{equation*}

Here, $f$ is a predictive model, $\mathbf{y}^*$ is the desired performance vector, and $\mathcal{L}_{\text{multi}}$ encodes a weighted loss across multiple objectives (e.g., runtime, energy, throughput). Instead of seeking a globally optimal configuration, \sysname returns a satisfying solution, one that meets all user constraints while trading off competing objectives. % reasonably.


%%%%%%%%%%%%%%%%%%%%%%%%
\noindent In contrast to counterfactuals--where an initial desirable full or partial configuration is known, %and outcomes are explored—
recommendation begins with a desired outcome and returns one or more feasible configurations that achieve it. The system searches over a constrained configuration space $\mathcal{C}$ for candidates that optimize one or more objectives.
If users provide constraints or thresholds across multiple performance metrics, the system formulates the query as a satisficing problem--identifying configurations that may not be globally optimal but lie within a trade-off region.

\textbf{How to use:} \tzi{@ankur -- please write an example of what would be the input by following my example at the end of section 3.4}

